First Results from the Dragonfly Ultrawide Survey: the Largest Eleven Quenched Diffuse Dwarf Galaxies in 3100 deg$^2$ with Spectroscopic Confirmation

The Dragonfly Telephoto Array employs a unique design to detect very large and diffuse galaxies, which might be missed with conventional telescopes. The Dragonfly Ultrawide Survey (DFUWS) is a new wide-field survey which will cover 10,000 deg$^2$ of the northern sky, and it provides an ideal dataset to find these large diffuse galaxies. From 3100 deg$^2$ of DFUWS data, we identified eleven large, low surface brightness galaxies as a pilot sample for spectroscopic follow-up. These are the largest galaxies in the examined area that appear smooth and isolated, with effective radii of 12"-27". Eight are below 24 $\mathrm{mag\,arcsec^{-2}}$ in central $g$-band surface brightness. Keck Cosmic Web Imager (KCWI) spectra of the diffuse light show that all eleven galaxies in this sample are quiescent, and seven qualify as ultra-diffuse galaxies (UDGs). Eight galaxies have distances between 15 and 30 Mpc, while the other three are in the Pegasus cluster at 50 Mpc. Their spectra show evidence of a $\sim 1$Gyr old stellar population in addition to an even older stellar population. The intermediate-age component is present in group and satellite galaxies but not in the Pegasus cluster UDGs. All galaxies in this sample are detected in both Dragonfly and Legacy imaging, and the sample partially overlaps with existing UDG catalogs. This pilot sample provides an excellent training set for our analysis of the upcoming full 10,000 deg$^2$ DFUWS data, from which we may expect to discover even larger, previously-unknown galaxies.

==> fig2set.tex <==
\figsetstart
\figsetnum{2}
\figsettitle{UW sample photometry}

\figsetgrpstart
\figsetgrpnum{2.1}
\figsetgrptitle{109}
\figsetplot{Autophot_Legacy_109_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.2}
\figsetgrptitle{117}
\figsetplot{Autophot_Legacy_117_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.3}
\figsetgrptitle{121}
\figsetplot{Autophot_Legacy_121_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.4}
\figsetgrptitle{16}
\figsetplot{Autophot_Legacy_16_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.5}
\figsetgrptitle{184}
\figsetplot{Autophot_Legacy_184_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.6}
\figsetgrptitle{258}
\figsetplot{Autophot_Legacy_258_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.7}
\figsetgrptitle{323}
\figsetplot{Autophot_Legacy_323_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.8}
\figsetgrptitle{54}
\figsetplot{Autophot_Legacy_54_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.9}
\figsetgrptitle{61}
\figsetplot{Autophot_Legacy_61_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.10}
\figsetgrptitle{68}
\figsetplot{Autophot_Legacy_68_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{2.11}
\figsetgrptitle{72}
\figsetplot{Autophot_Legacy_72_g.pdf}
\figsetgrpnote{Image data is from Legacy g-band; model for the galaxy is a Single sersic profile.}
\figsetgrpend

\figsetend

